Context-aware Adversarial Attack on Named Entity Recognition

In recent years, large pre-trained language models (PLMs) have achieved remarkable performance on many natural language processing benchmarks. Despite their success, prior studies have shown that PLMs are vulnerable to attacks from adversarial examples. In this work, we focus on the named entity recognition task and study context-aware adversarial attack methods to examine the model's robustness. Specifically, we propose perturbing the most informative words for recognizing entities to create adversarial examples and investigate different candidate replacement methods to generate natural and plausible adversarial examples. Experiments and analyses show that our methods are more effective in deceiving the model into making wrong predictions than strong baselines.

==> tables/adversarial_attack_results.tex <==
\begin{table*}[ht]
    \small
    \centering
    \setlength\tabcolsep{1pt}
    \renewcommand{\arraystretch}{1.0}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccccc}
        \toprule
        \multicolumn{3}{c}{\textbf{CoNLL03}} & \multicolumn{3}{c}{\textbf{OntoNotes5.0}} & \multicolumn{3}{c}{\textbf{WNUT17}} \\
        \cmidrule(lr){1-3} \cmidrule(lr){4-6} \cmidrule(lr){7-9}
        \bf F1 & \bf Sim. & \bf $\Delta$Perf. & \bf F1 & \bf Sim. & \bf $\Delta$Perf. & \bf F1 & \bf Sim. & \bf $\Delta$Perf. \\
        \toprule
        
        \toprule
        \multicolumn{9}{l}{\textbf{\textit{Perturbing 1 word in each sentence}}} \\
        \toprule
        \includegraphics[scale=0.15]{images/conll_f1_1.png} & \includegraphics[scale=0.15]{images/conll_text_similarity_1.png} & \includegraphics[scale=0.15]{images/conll_perf_1.png} & \includegraphics[scale=0.15]{images/ontonotes_f1_1.png} & \includegraphics[scale=0.15]{images/ontonotes_text_similarity_1.png} & \includegraphics[scale=0.15]{images/ontonotes_perf_1.png} &
        \includegraphics[scale=0.15]{images/wnut_f1_1.png} & \includegraphics[scale=0.15]{images/wnut_text_similarity_1.png} & \includegraphics[scale=0.15]{images/wnut_perf_1.png} \\
        
        \toprule
        \multicolumn{9}{l}{\textbf{\textit{Perturbing 2 words in each sentence}}} \\
        \toprule
        \includegraphics[scale=0.15]{images/conll_f1_2.png} & \includegraphics[scale=0.15]{images/conll_text_similarity_2.png} & \includegraphics[scale=0.15]{images/conll_perf_2.png} & \includegraphics[scale=0.15]{images/ontonotes_f1_2.png} & \includegraphics[scale=0.15]{images/ontonotes_text_similarity_2.png} & \includegraphics[scale=0.15]{images/ontonotes_perf_2.png} &
        \includegraphics[scale=0.15]{images/wnut_f1_2.png} & \includegraphics[scale=0.15]{images/wnut_text_similarity_2.png} & \includegraphics[scale=0.15]{images/wnut_perf_2.png} \\
        
        \toprule
        \multicolumn{9}{l}{\textbf{\textit{Perturbing 3 words in each sentence}}} \\
        \toprule
        \includegraphics[scale=0.15]{images/conll_f1_3.png} & \includegraphics[scale=0.15]{images/conll_text_similarity_3.png} & \includegraphics[scale=0.15]{images/conll_perf_3.png} & \includegraphics[scale=0.15]{images/ontonotes_f1_3.png} & \includegraphics[scale=0.15]{images/ontonotes_text_similarity_3.png} & \includegraphics[scale=0.15]{images/ontonotes_perf_3.png} &
        \includegraphics[scale=0.15]{images/wnut_f1_3.png} & \includegraphics[scale=0.15]{images/wnut_text_similarity_3.png} & \includegraphics[scale=0.15]{images/wnut_perf_3.png} \\
        
        \toprule
        \multicolumn{9}{l}{\textbf{\textit{Perturbing 4 words in each sentence}}} \\
        \toprule
        \includegraphics[scale=0.15]{images/conll_f1_4.png} & \includegraphics[scale=0.15]{images/conll_text_similarity_4.png} & \includegraphics[scale=0.15]{images/conll_perf_4.png} & \includegraphics[scale=0.15]{images/ontonotes_f1_4.png} & \includegraphics[scale=0.15]{images/ontonotes_text_similarity_4.png} & \includegraphics[scale=0.15]{images/ontonotes_perf_4.png} &
        \includegraphics[scale=0.15]{images/wnut_f1_4.png} & \includegraphics[scale=0.15]{images/wnut_text_similarity_4.png} & \includegraphics[scale=0.15]{images/wnut_perf_4.png} \\
        \toprule
        
        \multicolumn{9}{l}{\textbf{\textit{Perturbing 5 words in each sentence}}} \\
        \toprule
        \includegraphics[scale=0.15]{images/conll_f1_5.png} & \includegraphics[scale=0.15]{images/conll_text_similarity_5.png} & \includegraphics[scale=0.15]{images/conll_perf_5.png} & \includegraphics[scale=0.15]{images/ontonotes_f1_5.png} & \includegraphics[scale=0.15]{images/ontonotes_text_similarity_5.png} & \includegraphics[scale=0.15]{images/ontonotes_perf_5.png} &
        \includegraphics[scale=0.15]{images/wnut_f1_5.png} & \includegraphics[scale=0.15]{images/wnut_text_similarity_5.png} & \includegraphics[scale=0.15]{images/wnut_perf_5.png} \\
        \toprule
        \multicolumn{9}{c}{\includegraphics[scale=0.5]{images/legend.png}} \\
        \toprule
    \end{tabular}
    }
    \caption{The results of different adversarial attack methods on CoNLL03, OntoNotes5.0, and WNUT17 corpus. \textbf{RDM}, \textbf{PST}, \textbf{DEP}, \textbf{CHK}, \textbf{GDT} refer to random attack, POS-tagging attack, dependency-parsing attack, chunking attack, and gradient attack, respectively.}
    \label{tab: adversarial_attack_results}
\end{table*}





% \begin{table*}[ht]
%     \small
%     \centering
%     \setlength\tabcolsep{1pt}
%     \renewcommand{\arraystretch}{1.0}
%     \resizebox{\linewidth}{!}{
%         \begin{tabular}{ccccc}
%             \toprule
%             \multicolumn{5}{c}{\textbf{The Number of Candidates}} \\
%             \toprule
%             \bf 1 & \bf 2 & \bf 3 & \bf 4 & \bf 5 \\
%             \toprule
%             % \midrule
%             \multicolumn{5}{l}{\textbf{\textit{Using Synonym for Candidate Replacement}}} \\
%             \midrule
%             \includegraphics[scale=0.15]{images/conll_f1_1.png} & 
%             \includegraphics[scale=0.15]{images/conll_f1_2.png} & 
%             \includegraphics[scale=0.15]{images/conll_f1_3.png} & 
%             \includegraphics[scale=0.15]{images/conll_f1_4.png} & 
%             \includegraphics[scale=0.15]{images/conll_f1_5.png} \\
%             \midrule
%             \includegraphics[scale=0.15]{images/conll_text_similarity_1.png} & 
%             \includegraphics[scale=0.15]{images/conll_text_similarity_2.png} & 
%             \includegraphics[scale=0.15]{images/conll_text_similarity_3.png} & 
%             \includegraphics[scale=0.15]{images/conll_text_similarity_4.png} & 
%             \includegraphics[scale=0.15]{images/conll_text_similarity_5.png} \\
%             \midrule
%             \includegraphics[scale=0.15]{images/conll_perf_1.png} & 
%             \includegraphics[scale=0.15]{images/conll_perf_2.png} & 
%             \includegraphics[scale=0.15]{images/conll_perf_3.png} & 
%             \includegraphics[scale=0.15]{images/conll_perf_4.png} & 
%             \includegraphics[scale=0.15]{images/conll_perf_5.png}\\
%             \midrule
%             \multicolumn{5}{l}{\textbf{\textit{Using Synonym for Candidate Replacement}}} \\
%             \midrule
%             \includegraphics[scale=0.15]{images/wnut_f1_1.png} & 
%             \includegraphics[scale=0.15]{images/wnut_f1_2.png} & 
%             \includegraphics[scale=0.15]{images/wnut_f1_3.png} & 
%             \includegraphics[scale=0.15]{images/wnut_f1_4.png} & 
%             \includegraphics[scale=0.15]{images/wnut_f1_5.png} \\
%             \midrule
%             \includegraphics[scale=0.15]{images/wnut_text_similarity_1.png} & 
%             \includegraphics[scale=0.15]{images/wnut_text_similarity_2.png} & 
%             \includegraphics[scale=0.15]{images/wnut_text_similarity_3.png} & 
%             \includegraphics[scale=0.15]{images/wnut_text_similarity_4.png} & 
%             \includegraphics[scale=0.15]{images/wnut_text_similarity_5.png} \\
%             \midrule
%             \includegraphics[scale=0.15]{images/wnut_perf_1.png} & 
%             \includegraphics[scale=0.15]{images/wnut_perf_2.png} & 
%             \includegraphics[scale=0.15]{images/wnut_perf_3.png} & 
%             \includegraphics[scale=0.15]{images/wnut_perf_4.png} & 
%             \includegraphics[scale=0.15]{images/wnut_perf_5.png} 
%             \\
%             % \midrule
%             \toprule
%         \end{tabular}
%     }
%     \caption{The results of adversarial attack on different corpus.}
%     \label{tab: adversarial_attack_results}
% \end{table*}





% \begin{table*}[ht]
%     \small
%     \centering
%     \setlength\tabcolsep{1pt}
%     \renewcommand{\arraystretch}{1.0}
%     \resizebox{\linewidth}{!}{
%         \begin{tabular}{cccccccccc}
%             \toprule
%             \multicolumn{5}{c}{\textbf{F1 Score}} & \multicolumn{5}{c}{\textbf{Performance Decrease}} \\
%             \toprule
%             \bf 1 & \bf 2 & \bf 3 & \bf 4 & \bf 5 & \bf 1 & \bf 2 & \bf 3 & \bf 4 & \bf 5 \\
%             \toprule
%             \multicolumn{10}{l}{\textbf{\textit{Evaluation on CoNLL03}}} \\
%             \midrule
%             \includegraphics[scale=0.15]{images/conll_f1_1.png} & 
%             \includegraphics[scale=0.15]{images/conll_f1_2.png} & 
%             \includegraphics[scale=0.15]{images/conll_f1_3.png} & 
%             \includegraphics[scale=0.15]{images/conll_f1_4.png} & 
%             \includegraphics[scale=0.15]{images/conll_f1_5.png} \\
%             \midrule
%             \includegraphics[scale=0.15]{images/conll_text_similarity_1.png} & 
%             \includegraphics[scale=0.15]{images/conll_text_similarity_2.png} & 
%             \includegraphics[scale=0.15]{images/conll_text_similarity_3.png} & 
%             \includegraphics[scale=0.15]{images/conll_text_similarity_4.png} & 
%             \includegraphics[scale=0.15]{images/conll_text_similarity_5.png} \\
%             \midrule
%             \includegraphics[scale=0.15]{images/conll_perf_1.png} & 
%             \includegraphics[scale=0.15]{images/conll_perf_2.png} & 
%             \includegraphics[scale=0.15]{images/conll_perf_3.png} & 
%             \includegraphics[scale=0.15]{images/conll_perf_4.png} & 
%             \includegraphics[scale=0.15]{images/conll_perf_5.png}\\
%             \toprule
%             \multicolumn{5}{c}{\textbf{F1 Score}} & \multicolumn{5}{c}{\textbf{Performance Decrease}} \\
%             \toprule
%             \bf 1 & \bf 2 & \bf 3 & \bf 4 & \bf 5 & \bf 1 & \bf 2 & \bf 3 & \bf 4 & \bf 5 \\ \\
%             \toprule
%             \includegraphics[scale=0.15]{images/wnut_f1_1.png} & 
%             \includegraphics[scale=0.15]{images/wnut_f1_2.png} & 
%             \includegraphics[scale=0.15]{images/wnut_f1_3.png} & 
%             \includegraphics[scale=0.15]{images/wnut_f1_4.png} & 
%             \includegraphics[scale=0.15]{images/wnut_f1_5.png} \\
%             \midrule
%             \includegraphics[scale=0.15]{images/wnut_text_similarity_1.png} & 
%             \includegraphics[scale=0.15]{images/wnut_text_similarity_2.png} & 
%             \includegraphics[scale=0.15]{images/wnut_text_similarity_3.png} & 
%             \includegraphics[scale=0.15]{images/wnut_text_similarity_4.png} & 
%             \includegraphics[scale=0.15]{images/wnut_text_similarity_5.png} \\
%             \midrule
%             \includegraphics[scale=0.15]{images/wnut_perf_1.png} & 
%             \includegraphics[scale=0.15]{images/wnut_perf_2.png} & 
%             \includegraphics[scale=0.15]{images/wnut_perf_3.png} & 
%             \includegraphics[scale=0.15]{images/wnut_perf_4.png} & 
%             \includegraphics[scale=0.15]{images/wnut_perf_5.png} 
%             \\
%             % \midrule
%             \toprule
%         \end{tabular}
%     }
%     \caption{The results of adversarial attack on different corpus.}
%     \label{tab: adversarial_attack_results}
% \end{table*}

==> tables/case_study.tex <==
\begin{table*}[t!]
    \small
    \resizebox{\linewidth}{!}{
        \begin{tabular}{ll}
            \toprule
            \textbf{Method} & \textbf{Sentence} \\
            \toprule
            
            \midrule
            N/A 
            & \textbf{Original}: {[}Michael Jordan{]}\sub{PER} was a basketball player in {[}NBA{]}\sub{ORG} winning six championships with the {[}Chicago Bulls{]}\sub{ORG}. \\
            \midrule
            
            \midrule
            \multirow{3}{*}{Random} 
            & \textbf{Attack}: {[}Michael Jordan{]}\sub{PER} was a basketball player in {[}NBA{]}\sub{ORG} winning six championships with the {[}Chicago Bulls{]}\sub{ORG}. \\
            \cmidrule(lr){2-2}
            & \textbf{Synonym}: {[}Michael Jordan{]}\sub{PER} was a basketball player in {[}NBA{]}\sub{ORG} winning six championships with the {[}Chicago Bulls{]}\sub{ORG}. \\
            \cmidrule(lr){2-2}
            & \textbf{MLM}: {[}Michael Jordan{]}\sub{PER} was a basketball player in {[}NBA{]}\sub{ORG} winning six championships with the {[}Chicago Bulls{]}\sub{ORG}. \\
            \midrule
            
            \multirow{3}{*}{Random} 
            & \textbf{Attack}: {[}Michael Jordan{]}\sub{PER} was a basketball player in {[}NBA{]}\sub{ORG} winning six championships with the {[}Chicago Bulls{]}\sub{ORG}. \\
            & \textbf{Synonym}: {[}Michael Jordan{]}\sub{PER} was a basketball player in {[}NBA{]}\sub{ORG} winning six championships with the {[}Chicago Bulls{]}\sub{ORG}. \\
            & \textbf{MLM}: {[}Michael Jordan{]}\sub{PER} was a basketball player in {[}NBA{]}\sub{ORG} winning six championships with the {[}Chicago Bulls{]}\sub{ORG}. \\
            \midrule
            
            \multirow{3}{*}{Random} 
            & \textbf{Attack}: {[}Michael Jordan{]}\sub{PER} was a basketball player in {[}NBA{]}\sub{ORG} winning six championships with the {[}Chicago Bulls{]}\sub{ORG}. \\
            & \textbf{Synonym}: {[}Michael Jordan{]}\sub{PER} was a basketball player in {[}NBA{]}\sub{ORG} winning six championships with the {[}Chicago Bulls{]}\sub{ORG}. \\
            & \textbf{MLM}: {[}Michael Jordan{]}\sub{PER} was a basketball player in {[}NBA{]}\sub{ORG} winning six championships with the {[}Chicago Bulls{]}\sub{ORG}. \\
            \midrule
            
            \multirow{3}{*}{Random} 
            & \textbf{Attack}: {[}Michael Jordan{]}\sub{PER} was a basketball player in {[}NBA{]}\sub{ORG} winning six championships with the {[}Chicago Bulls{]}\sub{ORG}. \\
            & \textbf{Synonym}: {[}Michael Jordan{]}\sub{PER} was a basketball player in {[}NBA{]}\sub{ORG} winning six championships with the {[}Chicago Bulls{]}\sub{ORG}. \\
            & \textbf{MLM}: {[}Michael Jordan{]}\sub{PER} was a basketball player in {[}NBA{]}\sub{ORG} winning six championships with the {[}Chicago Bulls{]}\sub{ORG}. \\
            \midrule
            
            \multirow{3}{*}{Random} 
            & \textbf{Attack}: {[}Michael Jordan{]}\sub{PER} was a basketball player in {[}NBA{]}\sub{ORG} winning six championships with the {[}Chicago Bulls{]}\sub{ORG}. \\
            & \textbf{Synonym}: {[}Michael Jordan{]}\sub{PER} was a basketball player in {[}NBA{]}\sub{ORG} winning six championships with the {[}Chicago Bulls{]}\sub{ORG}. \\
            & \textbf{MLM}: {[}Michael Jordan{]}\sub{PER} was a basketball player in {[}NBA{]}\sub{ORG} winning six championships with the {[}Chicago Bulls{]}\sub{ORG}. \\
            \midrule
            
            \toprule
            
        \end{tabular}
    }
    \caption{
    Examples of data augmentation with data transformation for case study. The sentences are tagged with their corresponding entities in brackets (e.g., {[}NBA{]}\sub{ORG}).
    }
\label{tab: case_study}
\end{table*}

